Realizing Uncertainty-Aware Timing Stack in Embedded Operating System

Time awareness is critical to a broad range of emerging applications -- in Cyber-Physical Systems and Internet of Things -- running on commodity platforms and operating systems. Traditionally, time is synchronized across devices through a best-effort background service whose performance is neither observable nor controllable, thus consuming system resources independently of application needs while not allowing the applications and OS services to adapt to changes in uncertainty in system time. We advocate for rethinking how time is managed in a system stack. In this paper, we propose a new clock model that characterizes various sources of timing uncertainties in true time. We then present a Kalman filter based time synchronization protocol that adapts to the uncertainties exposed by the clock model. Our realization of a uncertainty-aware clock model and synchronization protocol is based on a standard embedded Linux platform.

==> Background.tex <==
\section{Quality of Time}
\label{sect:background}

There is a need to close the loop between the requirements and how well they are achieved.

We propose to introduce a complete timing stack inside an OS that handles time differently. Timelines is a key abstraction in this timing stack which is out of scope of this paper.

We advocate for a new way of thinking and provide a \textit{Quality of Time Stack} based on \textit{factored-coordination} approach in which time-aware applications express their willingness to share common time by binding to a \textit{timeline}. \textit{Timeline} is a virtual time-base established by devices in a timing subgroup. The key advantage with this approach is that a device can bind to multiple timelines, with different accuracy requirements; and the underlying system balances the synchronization needs with the system resources.

==> Evaluation.tex <==
\section{Evaluation}
\label{sect:eval}

==> Introduction.tex <==
\section{Introduction}
\label{sect:intro}

Awareness of time is critical to the reliability, security, and performance of distributed systems such as sensor networks, robot swarms, high frequency trading platforms, and global-scale databases. Technologies necessary for providing computing systems with an awareness of physical time such as precise network time synchronization protocols and stable clock sources, have seen rapid advances in recent years, and it is now possible to achieve low-nanosecond time synchronization between devices \cite{wr}. Despite this, commodity operating systems continue to manage time in an application-agnostic fashion; independent of applications' requirements on accuracy with which they need to know time, and without supplying any information about the achievable or current timing performance. Furthermore, technology trends such as wireless communications, power management, multi-core processors \cite{tsc}, and virtualization \cite{virtual} have introduced in the intervening system layers and additional sources of variations affecting application level knowledge of time. 

Traditional clock models do not cover all sources of uncertainties and synchronization protocols provide fixed accuracy with no visibility into the resultant uncertainty, even though it has proven that the knowledge of uncertainty in time enhances performance and reduces system complexity. For example, Google Spanner \cite{spanner} uses uncertainty in time to achieve external consistency of global database transactions. For real-time interactivity in cloud gaming, Outatime \cite{outatime} relaxes the stringent demands on frame speculation, provided the uncertainty in time is less than 100 milliseconds.

\begin{figure}[tbp]
\centering{}\includegraphics[width=6cm,height=5cm,keepaspectratio]{figs/overview.png}\protect\caption{QoT-aware Timing Stack}
\label{fig:arch-overview}
\end{figure}

We advocate for a new way of thinking about how time is managed across the system stack, and seek to transform the timing uncertainty in a computing system into a rich structure called, \textit{Quality of Time (QoT)} that is systematically measured, propagated and controlled throughout the system. This will shift the paradigm in time-aware applications from over-design to sense-and-adapt and make the applications QoT-aware. QoT captures metrics such as uncertainty and stability in time. Applications specify their QoT requirements, the operating system meets these requirements and exposes the achieved QoT back to the applications and services for them to adapt.
%QoT is a function of clock sources, network, and ambient conditions   
This form of closed-loop framework is shown in Figure \ref{fig:arch-overview}. The scope of this paper is only the highlighted control-loop in Figure \ref{fig:arch-overview}, where the applications and OS services' timing performance is controlled by predicting the state through the clock model.
%core module controls the performance of various services and applications based on the predicted state through the clock model.

Current clock models do not characterize all sources of uncertainties in time, and there is a need to learn and develop new models that expose uncertainties from all layers in a system stack i.e. from hardware, network stack and operating system etc. 
%we assert the need to learn and develop new clock models exposing various sources of uncertainties, and the usage of these models in the auto-tuning of synchronization protocols. 
Certain hardware capabilities have evolved over recent years to remove some sources of uncertainties. For example, MAC-layer time stamping for wireless transceivers greatly reduces timing uncertainty. Also, many radio transceivers now support interrupts at transmission and reception times. Certain processors have timer capture capability to precisely timestamp radio transceiver interrupts. Despite these hardware improvements, most timestamping mechanisms still suffer from timing jitter due to various uncertainties involved.

State-of-the-art synchronization protocols \cite{pulsesync}~\cite{ftsp} have taken clock drift as the only source of uncertainty in timing. In contrast, we point out some other sources of uncertainty that have an equal, if not more, effect on the timing performance. In this paper, we develop a clock model which takes into account different sources of timing uncertainties, such as clock drift, radio transceiver interrupt generation uncertainty, interrupt capture uncertainty, operating system uncertainty, and propagation delay. We conduct experiments to show the contribution of each and every source of timing uncertainty between master and slave nodes.
%To achieve this goal, we introduce timeline -- an operating system abstraction -- that provides a virtual common time base. Applications willing to share common time, bind to a timeline with the desired accuracy; the deviation the application is willing to tolerate with the timeline. These requirements are passed down to the operating system, which not only manages timelines but also keeps track of achieved QoT for each timeline. Our end-to-end \textit{timeline}-driven Quality of Time stack for Linux is shown in Figure \ref{fig:arch-overview}. The stack closes the loop between the timing requirements of applications, and how well the system is able or unable to meet their needs by propagating timing uncertainty back to the applications.
%\\The QoT stack also characterizes the timekeeping hardware capabilities e.g. oscillators and timestamping mechanisms, and exposes them as controllable and disciplinable clocks. 
In addition, we implement a Light Weight Kalman filter (LW Kalman) for time synchronization that learns and predicts its state by making use of the clock model. Certain control metrics such as clock source selection, clock rate, network topology and routing, time synchronization rate and signaling are used to tune the performance of the LW Kalman synchronization protocol. The scope of this paper however is only to show the effect of varying synchronization period on the LW Kalman's timing performance.

In the next section \ref{sect:model}, we describe our new clock model which fits the green \lq{\textit{Learn \& Model}}\rq~block in Figure \ref{fig:arch-overview}, and in section \ref{sect:tune-time-sync}, we explain the LW Kalman synchronization protocol that fits the red \lq{\textit{Control}}\rq~block in Figure \ref{fig:arch-overview}.

%The learn, predict and control loop constantly balances the application needs with the system resources.
%compensates for the uncertainties described above and achieves higher synchronization accuracy without sacrificing the limited resources available on most wireless devices. 
%This uncertainty-aware synchronization protocol is a proof of concept that the applications and services can adapt to the available resources and .
%In the following sections, we briefly explain the timeline abstraction and how it is managed in the OS. We then show how the OS extracts various sources of uncertainties and expose that to the applications. Finally we show that the applications can make use of these uncertainties to enhance their performance.

==> TimelineAbs.tex <==
\section{Quality of Time Architecture \& Stack}
\label{sect:tml}
We have implemented a complete stack for time management in Linux that is centered around the notion of timeline. The major components of the stack are shown in Figure \ref{fig:arch-overview}  Application developers make use of Timeline-based API to specify their QoT requirements which is then passed to the central component of the stack, the core in the kernel. The core is responsible for creation and management of timelines. On a per-timeline basis, the core initialize particular timekeeping hardware and services, extracts various sources of uncertainties from this hardware and services, and propagate these uncertainties to the applications. 
\\We will not go into the detailed implementation of the stack, instead we will briefly explain some key concepts on which the stack is built upon. This background is necessary for explaining how we introduce QoT in Linux.

\subsection{Timeline Abstraction}
\begin{figure}[tbp]
\centering
\includegraphics[width=6cm,height=5cm,keepaspectratio]{figs/Timeline-2.pdf}
\caption{Node 1 and 2 bind to 'Timeline' with an asymmetric accuracy around their true time $t_{1}$ and $t_{2}$ respectively}
\label{fig:timeline}
\end{figure}
A timeline is a virtual reference time base for all the nodes willing to share common time. A bunch of nodes in need to choreograph their tasks, bind to a common timeline with the desired $accuracy$. The $accuracy$ is an asymmetric error interval around the true time denoted as a $\{second,~attosecond\}$ tuple. The time at one node can deviate by no more than the $accuracy$ interval from all the other nodes bind to the same timeline. The timeline and its associated $accuracy$ is shown in Figure \ref{fig:timeline}.
The definition of timeline is completely decoupled from any node or fixed time reference. This enables us to escape the limitations of the static master-slave synchronization paradigm, and support applications that dynamically bind and unbind from timelines in an ad-hoc fashion. As a result, timeline based system is distributed, and enables adaptive groupings. 
\\Our Linux-based prototype implements the timeline abstraction as a character device, \textit{/dev/timelineX}, where $X$ corresponds to a unique identifier. The character device exposes the \textit{timeline reference} as a POSIX clock to userspace, which is disciplinable by a synchronization service. The timeline character device also exposes an Input-Output Control (ioctl) interface, for applications to bind/unbind to a timeline, specify/update their accuracy requirements, and read the timeline's reference time with an uncertainty estimate. In the Linux kernel, timelines are stored and ordered on a red-black tree which provides an $O(log(N))$ look-up time by string identifier.

\subsection{Timeline Management}
Timelines are ordered on a red-black tree as shown in Figure \ref{fig:timeline-mgmt} through $rb_node$ attribute, whereas, binding accuracies are stored in sorted linked lists through $list_head$ attribute in Linux. Of greatest importance to time management and synchronization is the ability to calculate the dominating accuracy for any given timeline, which is the highest accuracy across all associated bindings. We maintain linked lists of bindings, ordered by increasing accuracy against a single timeline node in the red-black tree. This way, we can efficiently track the dominating accuracy in a manner that is robust to the addition of a new binding, removal of an existing binding, and update of accuracy of an existing binding. In Figure \ref{fig:timeline-mgmt}, $Timeline~n$ has three bindings; and the last binding has the dominant accuracy requirement.

\begin{figure}[tbp]
\centering
\includegraphics[width=1\columnwidth]{figs/TML-MGMT.pdf}
\caption{Node 1 and 2 bind to 'Timeline' with an asymmetric accuracy around their true time $t_{1}$ and $t_{2}$ respectively}
\label{fig:timeline-mgmt}
\end{figure}
